Internet of things: a multiprotocol gateway as solution of the interoperability problem

One of the main challenges of the Internet of Things is the interoperability of highly heterogeneous devices, mainly in terms of the communication capabilities and network protocols used. As consequence, the interconnection model of the different devices involves an intermediary device, known as gateway. This gateway is a centralized element for the management of the devices that make up an IoT application. In addition, it is essential for the transmission of information to the Internet, especially when many IoT devices are not IP-based. This chapter describes a proposed model for an IoT gateway that allows the exchange of data through different wireless technologies and forwarding of such data to the Internet. The proposed gateway has important advantages such as: supporting for multiprotocol interconnectivity, the remote configuration of wireless nodes for sensor and actuators management; a flexible algorithm totranslate the data obtained by sensors into a uniform format for transmission to a cloud server; low energy consumption due to efficient data transfer over MQTT protocol. In order to demonstrate the usefulness of the developed gateway, a proof of concept test was implemented. The implemented scenario consists of 2 wireless nodes responsible for sensing environmental variables and transmitting data to the gateway node through different communication protocols. The obtained results show the feasibility for simultaneous data transmission from the remote wireless nodes to the gateway. Metrics on energy consumption in the devices are also presented.

==> Contents/acknow.tex <==
%%%%%%%%%%%%%%%%%%%%%%acknow.tex%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample acknowledgement chapter
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer %%%%%%%%%%%%%%%%%%%%%%%%%%

\extrachap{Acknowledgements}

Use the template \emph{acknow.tex} together with the Springer document class SVMono (monograph-type books) or SVMult (edited books) if you prefer to set your acknowledgement section as a separate chapter instead of including it as last part of your preface.



==> Contents/chapter_4.tex <==
%%%%%%%%%%%%%%%%%%%%% chapter.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\chapter*{Chapter 4. Advanced techniques for adaptive video streaming in SDNs}
\chapterauthor{Wilder Castellanos\footnote{Programa de Ingenier\'ia de Electr\'onica, Universidad de San Buenaventura sede Bogot\'a, Cra. 8H No. 172-20, Bogot\'a, Colombia. e-mail: wcastellanos@usbbog.edu.co}, Juan Gabriel Bustos\footnote{Programa de Ingenier\'ia de Electr\'onica, Universidad de San Buenaventura sede Bogot\'a, Cra. 8H No. 172-20, Bogot\'a, Colombia. e-mail: jbustos@academia.usbbog.edu.co} and Fran Wilson Sanabria\footnote{Programa de Ingenier\'ia de Electr\'onica, Universidad de San Buenaventura sede Bogot\'a, Cra. 8H No. 172-20, Bogot\'a, Colombia. e-mail: sfran@academia.usbbog.edu.co}}

%\chapauthor{Wilder Castellanos\footnote{Programa de Ingenier\'ia de Electr\'onica, Universidad de San Buenaventura sede Bogot\'a, Cra. 8H No. 172-20, Bogot\'a, Colombia. e-mail: wcastellanos@usbbog.edu.co}, Juan Gabriel Bustos\footnote{Programa de Ingenier\'ia de Electr\'onica, Universidad de San Buenaventura sede Bogot\'a, Cra. 8H No. 172-20, Bogot\'a, Colombia. e-mail: jbustos@academia.usbbog.edu.co} and Fran Wilson Sanabria\footnote{Programa de Ingenier\'ia de Electr\'onica, Universidad de San Buenaventura sede Bogot\'a, Cra. 8H No. 172-20, Bogot\'a, Colombia. e-mail: sfran@academia.usbbog.edu.co}}


\label{Chapter_4} % Always give a unique label
% use \chaptermark{}
% to alter or adjust the chapter heading in the running head
\abstract{
In the coming years a new management model of telecommunication networks will begin to be implemented. This model, known as Software Defined Networks, implies a radical change in the way networks are conceived today. Therefore, it is necessary to develop studies that allow to know this scenario and its implications during the transmission of different types of traffic. Especially, it is important to analyze the behavior of video traffic due to the significant increase of these flows through networks as well as to the massive use of new video services with ultra-high resolution formats. This fact also implies an enormous consumption of network resources like bandwidth. Likewise, the likelihood to impact on other traffic flows that coexist in the same network is increased caused by network congestion. Under these conditions the ability to adapt the video streams to the available resources of the network is an essential requirement in modern video services in order to prevent network congestion. Therefore, adaptive techniques for video transmission have become an important area of interest for researchers, technology providers and network operators.\newline\indent
This chapter briefly describes a study on software-defined networks and the tools necessary for video transmission on this type of networks. Among the aspects presented is the methodology used to establish the video transmission and the procedure to evaluate the quality obtained. A video transmission experiment is presented, which consists on the evaluation of adaptive transmission of video streams using adaptive techniques as MPEG/DASH and scalable coding. The experiments were carried out over a software-defined network topology in the MININET platform.
\newline\indent
\textit{Keywords:} Multimedia Delivery, Adaptive Video Streaming,  Software Defined Networks, DASH, SHVC}

\section{Introduction}
\label{sec:4.1}
With the inevitable implementation of SDNs (Software Defined Networks) by telecommunication network operators, it is necessary to start the evaluation of the multimedia flow transmission on this scenario. The new paradigm that involves SDNs includes the relocation of the control plane, currently located in network devices (routers and switches), to a single external element, the controller \cite{onf_2012}. This implies that instead of using distributed protocols such as BGP or OSPF, the controller is the software component responsible for routing and network control using standard management software.

In this new model for future networks and taking into account that video traffic is the predominant traffic through current networks, it is essential to develop experiments that study the optimization of the transmission of these flows so that increasing demand for video services can be satisfied, using network resources as efficiently as possible, without sacrificing the user quality experience.

Several aspects are relevant in this area, but mainly those that are related to providing users with video services and the video quality they demand, despite many times their connections do not have good communication quality management. In such scenarios, ability to adapt the video streams is essential. In this sense, multiple solutions have been proposed in recent years, such as more efficient encoders that allow to obtain high quality videos requiring less data.

This chapter describes the main concepts of software-defined networks, video coding and adaptive video transmission. In addition, we present a study where two techniques for adaptive transmission were analyzed: one corresponds to the use of MPEG/DASH (Dynamic Adaptive Streaming over HTTP) as an adaptation mechanism and the second consists in the use of the scalable coding standard SHVC (Scalable High Efficiency Video Coding). Also, we propose a methodology for the development of adaptive video transmission analysis on the MININET emulation platform \cite{lantz_2017}.

This chapter is organized as follows. Section 2 gives a brief forecast overview about the video services and the traffic problem in current networks. In Section 3 we give a brief introduction to the reference model for software defined networks. Section 4 summarizes the basic concepts on adaptive video streaming and then provides an overview on SHVC and DASH standards. The methodology and results of the performance evaluation of the adaptive methods are presented in Section 5. Finally, conclusions are presented in Section 6.

\section{Video Streaming: the digital revolution}
\label{sec:4.2}

The growing demand for streaming video services has resulted in a considerable increase in traffic through data networks. Some studies estimate that by 2022 82\% of network traffic will correspond to video traffic (see Fig.~\ref{ch4_fig:1}, which would be equivalent to every second, one million minutes of video being transmitted over the network \cite{Cisco_2019}. This figure includes all possible forms of IP video which includes Internet video, IP VoD, video conferencing, video-streamed gaming and video files exchanged through file sharing.  

\begin{center}
\includegraphics[scale=1.0]{Figures/ch_4_fig1_iptraffic.pdf}
\figcaption{Global IP traffic by application category \protect\cite{Cisco_2019}}
\label{ch4_fig:1}       % Give a unique label
\end{center}


%\begin{figure}[h!]
%\centering
%\includegraphics[scale=1.0]{Figures/ch_4_fig1_iptraffic.eps}
%\caption{Global IP traffic by application category \cite{Cisco_2019}}
%\label{ch4_fig:1}       % Give a unique label
%\end{figure}

Ericsson also forecasts a dramatic increase in video traffic in its “Mobility Report” \cite{ericsson2017}. This study foresees an increase in video traffic from mobile devices, from 16.59 ExaBytes/month (2018) to 97 ExaBytes/month in 2024. This means a 34 percent compound annual growth rate (CAGR). Globally, the total of video traffic in Internet will grow from 66.9 EB per month in 2017 to 282.3EB in 2022 (33\% CAGR) \cite{Cisco_2019}. This traffic represents 1.1 million of minutes of video transmitted every second.

This significant increase in video traffic is caused by new habits in the consumption of audiovisual content, since it is increasingly common to watch video contents in streaming mode, mainly due to the massive delivery of video on Internet and services such as Netflix, Hulu and YouTube. But not only streaming video services attract the attention of network operators.Video traffic growth is also driven mainly by: the increase of embedded video in many online applications, growth of video-on-demand (VoD) streaming services in terms of both subscribers and viewing time per subscriber, the evolving devices towards larger screens and higher resolutions and the new evolved 4G deployments that increase network performance. This fact is causing a change in the pattern of internet traffic that is going from being a traffic relatively steady to a more dynamic and bursty pattern traffic.

In particular, live Internet video has the potential to generate large amounts of traffic since it replaces the consumption of hours of traditional broadcast content. Live video already represents a 5 percent of Internet video traffic and will increase to reach 17 percent by 2022 \cite{Cisco_2019}. This means an increase of 15-fold in 5 years (72.7\% CAGR). Likewise, video surveillance traffic is of a very different nature than on-demand or live video and represents an upstream video traffic, uploaded continuously to the Internet. Fig.~\ref{ch4_fig:2} shows the growth of video traffic by subcategory. It is important to note that, long-form video will be 175 EB/month in 2022, 82.3\% of all Internet video traffic (including live and short-form video).

\begin{center}
\includegraphics[scale=0.83]{Figures/ch_4_fig_2_Internet_Video_Streaming.pdf}
\figcaption{Internet Video Streaming by Service Type \protect\cite{Cisco_2019}}
\label{ch4_fig:2}       % Give a unique label
\end{center} 
 
%\begin{figure}[h!]
%\centering
%\includegraphics[scale=1.0]{Figures/ch_4_fig_2_Internet_Video_Streaming.eps}
%\caption{Internet Video Streaming by Service Type \cite{Cisco_2019}}
%\label{ch4_fig:2}       % Give a unique label
%\end{figure}

With the arrival of the new generation wireless architectures, as well as the development of cameras and smartphones with the ability to record and play videos with ultra high definition (UHD) resolutions, user expectations are high as regards the possibility of transmitting higher quality video. This directly impact the network capacity since bit rate for a UHD video is about 18 Mbps, more than double the HD video bit rate and nine times more than Standard Definition (SD) video bit rate. And, UHD video will be 22\% of global Internet video traffic by 2022 (see Fig.~\ref{ch4_fig:3}). A trend that will increase with the arrival of 5G since users also expect immersive media and applications as well as 360-degree video and virtual/augmented reality \cite{mattos_2016}. 

\begin{center}
\includegraphics[scale=0.9]{Figures/ch_4_fig_3_Global_UHD.pdf}
\figcaption{Global UHD IP video traffic \protect\cite{Cisco_2019}}
\label{ch4_fig:3}       % Give a unique label
\end{center}

%\begin{figure}[h!]
%\centering
%\includegraphics[scale=1.0]{Figures/ch_4_fig_3_Global_UHD.eps}
%\caption{Global UHD IP video traffic \cite{Cisco_2019}}
%\label{ch4_fig:3}       % Give a unique label
%\end{figure}

This implies that efforts should be focused on the development and evaluation of new coding and compression methods, to produce videos that use the least amount of resources during the transmission and/or storage of that content.

Regarding video encoders, the most recently developed is the so-called H.265 / HEVC (High Efficiency Video Coding). This new standard promises to offer a 50\% better compression compared to the predecessor standard H.264, keeping the video with a reduced loss of quality. However, a greater complexity in compression algorithms is required  \cite{ye-kui_2016}. The H.265 Standard is a technique that allows you to respond to the challenge of optimizing UHD video transmission. This standard also has an extension for scalable video encoding SHVC (Scalable High Efficiency Video Coding), which promises to be a possible solution to UHD video transmission problems, providing adaptability in different topologies networks. Basically, SHVC encodes the video in several layers. This scalability feature allows the video to be adapted by transmitting only those layers that can be supported by network according to the available bandwidth estimation. This adaptation thus prevents network congestion and maintains a good level of video quality. In the same way, there is a technique called DASH (Dynamic Adaptive Streaming over HTTP) which consists of encoding a video with different qualities obtaining several representations of the same video. Each representation is divided into segments of short duration. A DASH Server will try to transmit those segments belonging to the representations of highest quality that can be supported by network.

\section{Software Define Networks}
\label{sec:4.3}

Today communication networks have increased their complexity caused by several reasons. Mainly due to the characteristics of new services and new consumption habits of users. For them mobility, security and a connection everywhere and every time are the priorities. It is difficult to overcome these challenges with the management model of the current networks. This is evidenced when services running on the network must be interrupted as soon as new services need to be implemented. In addition to the amazing increase in traffic from emergent services such as online games and virtual reality, new problems of adaptability and scalability are emerging. This has highlighted the need for a new management model for conventional networks.

Software Defined Networks involve a new vision on the management of communication networks. The main feature is the transfer of the control plane of physical devices to a new device, called a controller. This controller is a new network device in charge of manage or control a whole network. This fact allows network manager to configure devices such as switches, routers, network translators (NATs) or firewalls, using centralized software. In SDN model all networks devices can be programmed directly from the controller. In addition, more flexibility is obtained since network administrators can dynamically adjust traffic flows, in order to meet the changing needs of the services. Moreover, network managers can configure, manage and optimize network resources very quickly through dynamic and automated programs, which can be written by themselves. Since open standards are used, Software Defined Networks simplify the design and operation tasks of the networks, because instructions are provided by controllers rather than multiple vendor-specific devices and protocols \cite{onf_2012}.

\subsection{SDN Architecture}
\label{subsec:4.3.1}

In SDN model, network devices simply become specialized elements in packet forwarding tasks, which are executed according to a set of rules established by one or more controllers in control layer. These rules generally are predefined routines in application layer. On the other hand, the controller is a device located on a remote network and it communicates with the other network devices through a secure connection using a set of standardized commands \cite{jarraya_2014,muro_2016,xia_2015}.

As Fig.~\ref{ch4_fig:4} shows, in the reference model for SDN, the lower layer or infrastructure layer is where switching and routing devices (switches and routers) as well as other network devices are located. The control layer is made up of the SDN controller and it is separated from physical devices. Application Layer includes services or software applications that allow network managers or users executed specific tasks (such as bandwidth estimation and dynamic load balancing) over  the entire network.

\begin{center}
\includegraphics[scale=0.9]{Figures/ch_4_fig_4_Reference_Model.pdf}
\figcaption{Reference Model for SDNs}
\label{ch4_fig:4}       % Give a unique label
\end{center}

%\begin{figure}[h!]
%\centering
%\includegraphics[scale=0.7]{Figures/ch_4_fig_4_Reference_Model.eps}
%\caption{Reference Model for SDNs}
%\label{ch4_fig:4}       % Give a unique label
%\end{figure}

\section{Adaptive Video Transmission}
\label{sec:4.4}

Basically, video services are configured according to two main techniques: conventional video streaming and adaptive streaming. Conventional techniques include simple progressive download and real time streaming methods. In the progressive download technique, users request video content which is downloaded progressively into a local memory (buffer). According as the buffer has enough data the video starts to play. When playback rate overpasses the download rate, playback is stopped until more data is downloaded (see Fig.~\ref{ch4_fig:5}). Using a buffer some problems are solved, such as packet delay and the audio-video synchronization. Another conventional technique es the real time streaming, which consists on the establishment of a session between the video provider and users using a specialized network protocol \cite{castellanos_quality_2015}.

\begin{center}
\includegraphics[scale=0.6]{Figures/ch_4_fig_5_Progressive_download.pdf}
\figcaption{Progressive download technique}
\label{ch4_fig:5}       % Give a unique label
\end{center}

%\begin{figure}[h!]
%\centering
%\includegraphics[scale=0.6]{Figures/ch_4_fig_5_Progressive_download.eps}
%\caption{Progressive download technique}
%\label{ch4_fig:5}       % Give a unique label
%\end{figure}

However, conventional methods for video streaming are not flexible techniques since video content is delivered to the client using a constant bit rate over a fluctuating  connection. Therefore, if a communication link is suffering congestion, quality of the video is significantly degraded, as preliminary studies have revealed \cite{castellanos_quality_2015,gonzalez_2016}.

Some alternatives for conventional video delivery methods are the adaptive streaming techniques. These techniques allow video server to adapt the video quality that is provided to the client according to the available network resources. Therefore, algorithms for estimation of available resources, for example in terms of available bandwidth, have to be implemented. Some estimation mechanisms proposed can be  consulted in \cite{castellanos_available_2019,chaud_2015}. 

There are three techniques for adaptive video transmission proposed to reduce the problem that occurs with traditional transmission. One technique is the transcoding, which is a process converts a video to another using specific parameters during encode process in order to satisfy a certain bit rate \cite{gonzalez_2016}. This technique presents some problems due to permanent fluctuations in communication links which implies many adaptations of video flow. Therefore, a high consumption of resources in video server is carried out.

The second adaptive video streaming method is the flow switching \cite{bing_2015}. In this method a video is encoded several times obtaining many versions of the same video, each with different bit rates. Fig.~\ref{ch4_fig:6} shows an example of this method, where each video version is also divided into chunks of the same duration. A software program has to dynamically choose the video version that matches the bandwidth available in the network. Although this technique minimizes processing costs, storage and transmission requirements must be considered because the same video content is encoded several times \cite{gonzalez_2016}. An example of this technique is the MPEG-DASH standard. This standard defines that the client has exclusively the control of the adaptive streaming process \cite{bing_2015}. The DASH client is responsible for requesting the server information required to carry out the video transmission. For this, videos must be encoded using the DASH standard. When a video is encoded in DASH, a file called manifest (or mpd) is generated, which must be stored on the server. The different representations of the video are also stored there. These representations are different versions of the original video, each version with different quality. These representations of the video are subdivided into segments (chunks) of a short duration. In this way, if network resources are very restrictive, DASH client can request the transmission of segments of the lowest quality representation to server.  Segments of the representation of best quality can be transmitted as more resources are available. A description of the video transmission using DASH is given in Fig.~\ref{ch4_fig:7}. As can be seen in this figure, several representations of the same video are stored on the HTTP server. Each representation has a specific bit rate and is composed of several segments. The mpd file is sent from server to client, so that it knows the configuration of the different representations. Therefore, client requests the suitable representation according to its available resources.

\begin{center}
\includegraphics[scale=1.0]{Figures/Ch_4_Fig6_flow_switching.pdf}
\figcaption{Flow switching method}
\label{ch4_fig:6}       % Give a unique label
\end{center}

%\begin{figure}[h!]
%\centering
%\includegraphics[scale=1.0]{Figures/Ch_4_Fig6_flow_switching.eps}
%\caption{Flow switching method}
%\label{ch4_fig:6}       % Give a unique label
%\end{figure}

\begin{center}
\includegraphics[scale=0.7]{Figures/ch_4_fig_7_DASH_Video_Transmission.pdf}
\figcaption{DASH Video Transmission \protect\cite{kua_2017}}
\label{ch4_fig:7}       % Give a unique label
\end{center}

%\begin{figure}[h!]
%\centering
%\includegraphics[scale=0.7]{Figures/ch_4_fig_7_DASH_Video_Transmission.eps}
%\caption{DASH Video Transmission \cite{kua_2017}}
%\label{ch4_fig:7}       % Give a unique label
%\end{figure}

The third technique for adaptive video streaming uses Scalable Video Coding, which has attracted notable interest by researchers in order to improve video delivery over hybrid networks \cite{castellanos_improving_2018} and wireless networks \cite{castellanos_svceval-ra_2017}. The most recent standard for scalable video coding is known as SHVC (Scalable High Efficiency Video Coding). A video encoded with SHVC standard has a layered structure where the layers store information about different temporal, spatial or quality representations. The base layer corresponds to the more basic representation of the video. To this basic version of the video can be added several layers, known as enhancement layers. One or more enhancement layers increase the frame size, frame rate or video quality. The layered scheme of SHVC allow video server to send only layer data that can be supported by communication network. Fig.~\ref{ch4_fig:8} illustrates an example of the basic operation of the scalable transmission of a video containing three layers, each layer with different quality.

\begin{center}
\includegraphics[scale=0.43]{Figures/Ch_4_Fig8_scalable.pdf}
\figcaption{Scalable Video Transmission}
\label{ch4_fig:8}       % Give a unique label
\end{center}

%\begin{figure}[ht!]
%\centering
%\includegraphics[scale=0.43]{Figures/Ch_4_Fig8_scalable.eps}
%\caption{Scalable Video Transmission}
%\label{ch4_fig:8}       % Give a unique label
%\end{figure}

\section{SHVC and DASH: tools and comparative evaluation}
\label{sec:4.5}
After understanding the operation and advantages of the DASH and SHVC standards in adapting video streams during a transmission, results of evaluating video transmission with these two methods are now described. This study has two objectives. On the one hand, to identify the main elements that make up an SDN and those components required to perform video traffic evaluations on this type of networks. And, on the other hand, to carry out a performance evaluation of adaptive video transmission over software-defined networks using DASH and SHVC techniques.

In experiments, a same video was transmitted using the two adaptive techniques (DASH and SHVC) in order to analyze which of them have better performance. In addition to adaptive streams, a video encoded in H.265 (non-adaptive) was also transmitted in order to determine the advantage of adaptive techniques respect to traditional streaming method.

The network scenario used in this evaluation is the NSFNET-14 network (National Science Foundation's Network). This network corresponds to a national optical network with 14 nodes, located in the United States and destined for research and education.

\subsection{Proposed methodology}
\label{subsec:4.5.1}
The methodology followed in the experiments described in this chapter is similar to the methodology of the previous experiments. 

\begin{center}
\includegraphics[scale=0.9]{Figures/Ch_4_Fig9_methodology.pdf}
\figcaption{Methodology for the development of the experiments}
\label{ch4_fig:9}       % Give a unique label
\end{center}

%\begin{figure}[ht!]
%\centering
%\includegraphics[scale=0.8]{Figures/Ch_4_Fig9_methodology.eps}
%\caption{Methodology for the development of the experiments}
%\label{ch4_fig:9}       % Give a unique label
%\end{figure}

Basically, there is a first preprocessing stage, in which the original video is encoded. In these experiments a testing video of 1200 frames was generated concatenating the well-known video sequences “mobile.yuv” with CIF resolution (352x288 pixeles) (see Fig.~\ref{ch4_fig:10}). This video was encoded with three tools in order to obtain three videos with different formats: H.265, DASH and SHVC. The H.265 coding was performed with the HM encoder; DASH video was generated with HM encoder to obtain an H.265 stream and then with MP4Box program to generate the DASH segments. Finally, SHM software was used to obtain the encoded video in SHVC. In the case of the H265 encoding, the video has a level of compression (CRF, Constant Rate Factor) of 20, in DASH there are three representations with three different levels of compression CRF of 20, 30 and 40, each with eight segments of 10 seconds of duration. SHVC Video has two layers, one with CRF of 20 and another of 40. It is important to remark that SHM encoder (official encoder for SHVC) allows maximum coding with 2 layers, therefore it was not possible to obtain a video with more scalability layers.

\begin{center}
\includegraphics[scale=0.3]{Figures/Ch_4_Fig10_example.png}
\figcaption{Example frame of mobile.yuv}
\label{ch4_fig:10}       % Give a unique label
\end{center}

%\begin{figure}[ht!]
%\centering
%\includegraphics[scale=0.5]{Figures/Ch_4_Fig10_example.png}
%\caption{Example frame of mobile.yuv}
%\label{ch4_fig:10}       % Give a unique label
%\end{figure}

The second step of the methodology is the emulation of the network scenario and the independent transmission for each of the three videos. Thus, a video was received for each case. During video transmissions, traffic statistics of the video packets were recorded, which allowed that network performance be analyzed later. The network scenario, called NSFNET-14, was implemented in MININET, and consists of 14 nodes (see Fig.~\ref{ch4_fig:11}). The client and the server are located at opposite ends of the network, with host h1 being the client and h2 the server, as shown in Fig.~\ref{ch4_fig:11}. Bandwidth fluctuations were programmed as follows. Initially capacity of the client link is 400Kbps, then increases to 1200Kbps, then increases again to 2000Kbps and finally decreases to 1200Kbps. These bandwidth variations were made in the following instants of time: 3 seconds after the emulation starts, 14 seconds and 25 seconds, respectively. In addition, for this topology it was necessary to establish and configure routes (bidirectional routes) between client node and the server. This route management was done using the OpenFlow protocol.

\begin{center}
\includegraphics[scale=1.0]{Figures/Ch_4_Fig11_NSFNET14.pdf}
\figcaption{NSFNET-14 network topology}
\label{ch4_fig:11}       % Give a unique label
\end{center}

%\begin{figure}[ht!]
%\centering
%\includegraphics[scale=1.0]{Figures/Ch_4_Fig11_NSFNET14.eps}
%\caption{NSFNET-14 network topology}
%\label{ch4_fig:11}       % Give a unique label
%\end{figure}

The last methodology stage was the post-processing. In this stage the received videos were decoded to YUV format to compare them with the original RAW video in order to measure the video quality in terms of PSNR (Peak Signal Noise Rate). PSNR is an objective metric used to estimate the image quality of a video in comparison with its original version. Therefore, the calculation of the PSNR gives us a clear quantification of the distortion suffered by the video. This metric is one of the most used to evaluate the quality of a video after its transmission over a network. Equation (1) shows the definition of the PSNR \cite{bing_2015}.

\begin{equation}
    PSNR=10 \cdot log_{10}( \dfrac{255^2}{MSE}) \ \ \ \ \textup{where,}
\end{equation}

\begin{equation}
    MSE=\frac{1}{N \cdot M} \sum^{M-1}_{m=0} \sum^{N-1}_{n=0} |I_{org} (m,n) - I_{rec} (m,n)|^2
\end{equation}


Where, Iorg is the original frame and Irec is the frame received after transmission; M, N is the size of the frame and MSE is the mean square error. According to (2), the PSNR can be understood as the comparison pixel by pixel, of each frame contained in the two videos (original and received). Therefore, the PSNR metric is a value that indicates the distortion experienced by received video regarding the original.

Other network performance metrics as delay, throughput and percentage of lost packets were calculated. To obtain that metrics a traffic capture was performed during video transmission. This capture of traffic was carried out using TCPDUMP software. However, in order to automate the data processing of traffic records, a Python program was implemented. This program integrates other scripts programmed in different programming languages such as Perl and Awk, as well as native Linux applications such as Bash, Grep, Sed, Join, Sort and Gnuplot. For additional information on the source code and operation of the program, can be consulted \cite{bustos_2019}.

\subsection{Simulation results}
\label{subsec:4.5.2}

In this section we present the results obtained from the network emulation and transmission of the three videos. It is important to note that the transmission of H.265, DASH and SHVC videos, was performed five times, in order to obtain statistically significant results. Therefore, each data points in figures represents an average of at least five runs with identical traffic.

Quality of the received videos is shown in Fig.~\ref{ch4_fig:12}, where PSNR of the three video formats is compared. The average PSNR for each video was also calculated, obtaining a PSNR of 11.35 dB, 27.67 dB and 31.01 dB for H265, SHVC and DASH videos, respectively.

\begin{center}
\includegraphics[scale=0.6]{Figures/Ch_4_Fig12_averagePSNR.pdf}
\figcaption{Average PSNR of transmissions made on the NSFNET-14 topology.}
\label{ch4_fig:12}       % Give a unique label
\end{center}

%\begin{figure}[ht!]
%\centering
%\includegraphics[scale=0.6]{Figures/Ch_4_Fig12_averagePSNR.eps}
%\caption{Average PSNR of transmissions made on the NSFNET-14 topology.}
%\label{ch4_fig:12}       % Give a unique label
%\end{figure}

The PSNR curves allow to identify quality changes caused by the variation of the available bandwidth. Also, in Fig.~\ref{ch4_fig:12} the adaptation of the SHVC and DASH flows can be observed. On the contrary, using H265 encoding a very low PSNR (low quality) was obtained. The adaptability of DASH and SHVC streams allows user to obtain a higher video quality compared to quality of the H.265 stream (non-adaptive). The PSNR difference of H.265 in relation to DASH is 19.66 dB, and 16.32 dB in relation to SHVC, which shows that adaptive flows provide a significant improvement in quality.

In order to show that PSNR differences are reflected in video quality perceived by user, Fig.~\ref{ch4_fig:13} shows the image quality of a frame as an example. Fig.~\ref{ch4_fig:13} (a) shows the frame 510 of video encoded in H.265 and Fig.~\ref{ch4_fig:13}(b) shows the heat map resulting from the comparison with the same frame of the original video. Similarly, in Fig.~\ref{ch4_fig:13}(c) and Fig.~\ref{ch4_fig:13}(e) illustrate frames 510 of SHVC and DASH videos, respectively. The respective heat maps for these flows are also shown in Fig.~\ref{ch4_fig:13}(d) and Fig.~\ref{ch4_fig:13}(f). Red pixels in heat maps represent areas with high information losses (i.e. a low PSNR), while blue pixels represent best image quality. In Figure 13 below each heat map the PSNR value is shown. In this case, the frame with the lowest PSNR is correspond to H.265 video.

\begin{center}
\includegraphics[scale=0.6]{Figures/Ch_4_Fig13_image.png}
\figcaption{Image quality of frame 510 for the three types of video.}
\label{ch4_fig:13}       % Give a unique label
\end{center}

%\begin{figure}[ht!]
%\centering
%\includegraphics[scale=0.6]{Figures/Ch_4_Fig13_image.png}
%\caption{Image quality of frame 510 for the three types of video.}
%\label{ch4_fig:13}       % Give a unique label
%\end{figure}

Network traffic behavior was also assessed throughout the measurement of throughput metric. In Fig.~\ref{ch4_fig:14} is depicted the variation of the total network throughput achieved while videos were transmitted from server to client node. Also, the variation of link capacity is shown in that Figure. The average values of the throughput for each case were: 1.22 Mbps, 243.5 Kbps and 377.5 Kbps, for H265, SHVC and DASH, respectively.

By analyzing curves in Fig.~\ref{ch4_fig:14}, it can be observed that in the cases of SHVC and DASH network is not saturated, since only packets belonging SHVC layer or DASH representation that can be supported, were transmitted over the network. Regarding H.265 video, server always tries to transmit video packets at highest quality, even when link bandwidth is more restrictive. Therefore, network is prone to congestion degrading the overall flow transmissions.

\begin{center}
\includegraphics[scale=0.6]{Figures/Ch_4_Fig14_averageThroughput.pdf}
\figcaption{Throughput achieved for each video transmission.}
\label{ch4_fig:14}       % Give a unique label
\end{center}

%\begin{figure}[ht!]
%\centering
%\includegraphics[scale=0.6]{Figures/Ch_4_Fig14_averageThroughput.eps}
%\caption{Throughput achieved for each video transmission.}
%\label{ch4_fig:14}       % Give a unique label
%\end{figure}

Network congestion for the H.625 flow can be confirmed if the end to end delay is analyzed. Packet delay values for each video stream are presented in Fig.~\ref{ch4_fig:15}. Average values for the packet delay were calculated, obtaining 1.3417, 0.0972 and 0.0995 seconds, for H265, SHVC and DASH, respectively. As can be observed, packets of adaptive flows presented a low delay. This means that network congestion was avoided. However, for H265 flow, a high delay affected its packets and this an indicator of network congestion. These high delay values influenced the perceived quality of the H.265 video since a smooth reproduction of the video was not obtained.

\begin{center}
\includegraphics[scale=0.6]{Figures/Ch_4_Fig15_averageDelay.pdf}
\figcaption{Average end to end delay for each video flow.}
\label{ch4_fig:15}       % Give a unique label
\end{center}

%\begin{figure}[ht!]
%\centering
%\includegraphics[scale=0.6]{Figures/Ch_4_Fig15_averageDelay.eps}
%\caption{Average end to end delay for each video flow.}
%\label{ch4_fig:15}       % Give a unique label
%\end{figure}

On the other hand, throughput achieved for each video flows can be confirmed counting the number of sent packets during video transmissions. Table~\ref{ch4_tab:1} shows that using SHVC fewer packets were transmitted, only 1.155 packets. DASH flows used 1718 packets and with the highest amount of sent packets, the H265 video. The last metric obtained related to the network performance was the packet loss, which was represented in terms of percentage. This metric considers the packets sent by video server and those received by client host, calculated values are shown in Table~\ref{ch4_tab:1} and depicted in Fig.~\ref{ch4_fig:16}.

\begin{table}[ht!]
    \centering
\caption{Packet statistics in video transmissions}
\label{ch4_tab:1}
    \begin{tabular}{|c|c|c|c|c|}
         \hline
 & Sent Packets & Received Packets & Lost Packets & Percentage of lost packets \\
\hline
H265 & 6.421,6 & 6.329,0 & 92,9 & 1.44\% \\
\hline
SHVC & 1.155 & 1.142,2 & 12,8 & 1,1\% \\
\hline
DASH & 1.718,2 & 1.703,2 & 15 & 0.87\%\\
\hline
    \end{tabular}
\end{table}

\begin{center}
\includegraphics[scale=0.6]{Figures/Ch_4_Fig16_percentageLoss.pdf}
\figcaption{Percentage of lost packets.}
\label{ch4_fig:16}       % Give a unique label
\end{center}

%\begin{figure}[ht!]
%\centering
%\includegraphics[scale=0.6]{Figures/Ch_4_Fig16_percentageLoss.eps}
%\caption{Percentage of lost packets.}
%\label{ch4_fig:16}       % Give a unique label
%\end{figure}

Although the number of lost packets is low for the three streams, the H.265 stream experienced the highest amount of packets loss. A low percentage of lost packets and a low delay (as in the case of DASH and SHVC) means a better adaptation of the traffic flow to the maximum link capacity. 

\section{Conclusions}
\label{sec:4.6}

Initially in this chapter we present important forecasts about the massive explosion of the video services and the consequent increase in the real time traffic on the current network infrastructures. Then, the main aspects concerning video transmission over software defined networks were analyzed. Particularly, techniques for adaptive video streaming were presented since these techniques are the most suitable methods for multimedia content delivery over networks with limited available resources. 

One of the most important contributions of this chapter is the methodology and  the tools proposed for developing video transmission experiments over SDNs. Using this tool set we carried out a study on adaptive video streaming with three different encoding standards: H.265, SHVC and DASH. These standards are the most recent for video coding and they are the encoding standards that will be used in near future for developing the next generation of UHD (Ultra High Definition) video services.

Regarding video transmission evaluation on SDNs, adaptive techniques like DASH and SHVC outperform H.265 in terms of quality of received video, throughput and video packet delay. Particularly, DASH proved to be an efficient adaptation technique since it allowed to obtain not only higher quality videos, but also experienced low delay and low packet losses.

Using SHVC good results also were obtained. Although the ability of SHVC to effectively adapt to the capacity of the link could be checked, its current limitation of only being able to add one improvement layer makes it less flexible. The great advantage of SHVC is that only one version of the video is stored on server, while several versions of the same video must be stored with DASH, which significantly increases the disk space used.

The worst results obtained were reached by transmitting the video encoded only with H.265 standard, without any adaptive technique. Although more video information is sent with H265, the lack of adaptation to variations in available bandwidth of the data network causes network congestion. Therefore, the delay and packet losses significantly increase, obtaining a received video with very low quality.

On the contrary, with adaptive techniques, although not all information contained in the original video is sent, a better quality of experience is obtained by user. This fact that can be demonstrated evaluating the PSNR.

On the other hand, throughput measurements show that adaptive techniques make more efficient use of bandwidth, preventing congestion network and avoiding affect other simultaneous traffic flows. This situation also allows delay and packet loss to be noticeably smaller, compared to transmissions where adaptive video techniques are not used.
Finally, we can conclude that adaptive techniques are absolutely essential for the transmission of current high-performance video services, both in conventional networks and in the new model defined by the SDN.

\section*{Acknowledgements}
 This work is supported by the Universidad de San Buenaventura under the project “PERSEO: Plataforma para Evaluar los Sistemas de vidEO de las aplicaciones de próxima generación” (CBI 013-008)

==> chapter_5.tex <==
%%%%%%%%%%%%%%%%%%%%% chapter.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% sample chapter
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%\motto{Use the template \emph{chapter.tex} to style the various elements of your chapter content.}

\chapauthor{Wilder Castellanos
\footnote{Programa de Ingenier\'ia Electr\'onica, Universidad de San Buenaventura sede Bogot\'a, Cra. 8H No. 172-20, Bogot\'a, Colombia. e-mail: wcastellanos@usbbog.edu.co} 
Jose Macias
\footnote{Programa de Ingenier\'ia Electr\'onica, Universidad de San Buenaventura sede Bogot\'a, Cra. 8H No. 172-20, Bogot\'a, Colombia. e-mail: jmacias@academia.usbbog.edu.co}, 
Harold Pinilla 
\footnote{Programa de Ingenier\'ia Electr\'onica, Universidad de San Buenaventura sede Bogot\'a, Cra. 8H No. 172-20, Bogot\'a, Colombia. e-mail: hpinilla@academia.usbbog.edu.co}, 
Jose David Alvarado
\footnote{Programa de Ingenier\'ia Electr\'onica, Universidad de San Buenaventura sede Bogot\'a, Cra. 8H No. 172-20, Bogot\'a, Colombia. e-mail: jalvarado@usbbog.edu.co}. 
}

\chapter{Internet of things: a multiprotocol gateway as solution of the interoperability problem}
\label{Chapter_5} % Always give a unique label
% use \chaptermark{}
% to alter or adjust the chapter heading in the running head

\abstract{In the coming years, the interconnection of a large number of devices is expected, which will lead to a new form of interaction between the real and the virtual world. In this promising scenario, known as the Internet of Things (IoT), it is expected that different objects, such as sensors, industrial robots, cars, appliances, etc., will be continuously connected to the Internet. One of the main challenges of the Internet of Things is the interoperability of highly heterogeneous devices, mainly in terms of the communication capabilities and network protocols used. As consequence, the interconnection model of the different devices involves an intermediary device, known as gateway. This gateway is a centralized element for the management of the devices that make up an IoT application. In addition, it is essential for the transmission of information to the Internet, especially when many IoT devices are not IP-based.
This chapter describes a proposed model for an IoT gateway that allows the exchange of data through different wireless technologies and forwarding of such data to the Internet. The proposed gateway has important advantages such as: supporting for multiprotocol interconnectivity; the remote configuration of wireless nodes for sensor and actuators management; a flexible algorithm to translate the data obtained by sensors into a uniform format for transmission to a cloud server; low energy consumption due to efficient data transfer over the MQTT protocol. In order to demonstrate the usefulness of the developed gateway, a proof-of-concept test was implemented. The implemented scenario consists of 2 wireless nodes responsible for sensing environmental variables and transmitting data to the gateway node through different communication protocols. The obtained results show the feasibility for simultaneous data transmission from the remote wireless nodes to the gateway. Metrics on energy consumption in the devices are also presented.}
\textit{Keywords:} Internet of Things, Wireless Sensor Network, Multiprotocol gateway, MQTT.

\section{The Internet of Things: perspectives and challenges}
\label{sec:5.1}

The Internet of Things is a new technological paradigm that promotes the vision of a global network of devices capable of interacting with each other \cite{Gubbi2013,Lee2015}. In IoT scenarios these all devices acquire information, process it and share it. Current studies on the ecosystem associated with IoT estimate 127 new IoT devices connect to the Internet every second \cite{Lucero2016}. This implies that in 2022 the M2M (Machine-to-Machine) traffic could reach 25ExaBytes per month (7\% of all Global internet traffic) \cite{Cisco2019}. This significant increase in traffic between devices will be due to the significant growth in the number of machines connected. Cisco estimates that M2M connections will grow from 6.1 Billion in 2017 to 14.6 billion by 2022 (Fig \ref{ch5_fig:1}). Connected home applications such as connected household appliances, video surveillance, home automation and tracking applications, will represent 48 \%, of the total M2M connections by 2022 \cite{Cisco2019}. 
% For figures use
%
\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=1.0]{Figures/Fig1_M2MConections}
\caption{Number of M2M connections per year}
\label{ch5_fig:1}       % Give a unique label
\end{figure}

From the point of view of the economy, the effect of the IoT incursion will also be considerable. In this sense, in the report titled “Global Internet of Things (IoT) market: Global market analysis, insights and forecast, 2019-2026” \cite{FBI2019} the global market of was valued at US\$ 190 Billion in 2018 and is estimated to reach \$ 1111.3 Billion by 2026 \cite{USAIDCC2019}. Some reports also predict the global market of IoT will expand at a CAGR (Compound annual growth rate) of 24.7 \% during the next 5 years. For example, the market for wearable devices is expected to grow to 162.9 million devices by the end of 2020, mainly led by Fitness trackers. Smart homes are also an important area in IoT, according to Business Insider forecasts (Meola, 2018), they will grow from 82 million in 2015 to 193 million in 2020 this will represent almost US\$58.7 Billion in 2020 \cite{Statista2018}. In transportation area, will In the area of transport, 220 million connected cars are estimated in 2020, approximately 190 million of cars more than in 2015 \cite{Meola2018}. In the agriculture sector, growth in the number of IoT devices is estimated from 30 million in 2015 to 75 million in 2020. In Banking and Financial Services market, the IoT will grow from US\$0.17 Billion in 2017 to 2.03 Billion by 2023. These forecasts show a new mode of interaction with the physical world, inspired by the idea of ubiquity, where all the devices that surround us (sensors, cars, refrigerators, thermostats, industrial robots, tables, smartphones, etc.) can be connected to Internet anytime and anywhere. 

However, several challenges must be overcome. Mainly those related to security and interoperability issues of the devices. Interoperability is not a minor issue due to the high degree of heterogeneity of the available IoT devices. This heterogeneity is mainly accentuated in communication capabilities (protocols, technologies and hardware) of the IoT components. Some figures that illustrate the magnitude of the problem are provided by some preliminary studies \cite{Alvarado2018, alvarado_2017}. For example, about 10 different communication standards for IoT systems have been recently identified. Some IoT protocols are: Bluetooth, WiFi, ZigBee, 6LoWPAN, LoRa and Sig-Fox. This implies a difficulty during the implementation of a real system where it is necessary to guarantee full interoperability. In particular, the interoperability requirement is one of the major challenges that must be addressed for the integration and development of new IoT platforms \cite{Al-Fuqaha2015}. Some studies estimates that about 40\% of the potential benefits of IoT could be lost due to the lack of interoperability between different devices \cite{Manyika2015}. Solving the interoperability problem will eliminate so-called closed ecosystems \cite{Desai2015}, obtaining the true value of IoT, that is, data that is acquired and transmitted through the interaction between devices \cite{Evans2011}. One possible solution is the integration of a multiprotocol IoT gateway capable of performing data exchange with several wireless nodes, through different network protocols such as WiFi, Bluetooth and Zigbee. An IoT gateway also establishes a connection to a server on the Internet to perform data analytics. 

In order to show how an IoT gateway should be implemented, we proposed a gateway architecture that enables data communication using different network protocols. The evaluation of the proposed gateway was carried out through a use case, which consisted of the implementation of two wireless nodes, each with 6 sensors. Data readings are transmitted from wireless nodes to gateway through WiFi, Bluetooth and Zigbee. Gateway performance was analyzed based on the measurement of the percentage of CPU usage and free memory, as well as the analysis of the throughput reached in each network interface.	

\section{IoT Gateway: bridge device between sensor network and cloud platforms}
\label{sec:5.2}

In general terms, a gateway is a device that allows communication between networks with different protocols. This task required to convert the formats of the received data to the structure of the destination protocol. In the scenario of IoT, a gateway is a device that supports communications with different communication protocols and data formats. Therefore, an IoT gateway allows to interconnect multiple types of sensors as well as the aggregation of several IoT nodes with other segments of the network or with Internet. This is the main objective of a gateway, to serve as a bridge between several network domains with a public network or the Internet, solving the problem of heterogeneity between these domains \cite{Zachariah2015}. At the same time, a gateway becomes an ideal device for network management functions, since while exchanging messages with the sensor nodes, it can map the network and establish a comprehensive knowledge of the network. 

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=1.0]{Figures/Fig2_MainIoTGateway}
\caption{Main characteristics for an IoT Gateway}
\label{ch5_fig:2}       % Give a unique label
\end{figure}

The different types of gateways for IoT can be classified as passive, semi-automatic and fully automatic. In passive gateways new IoT devices, as sensor nodes, must be configured manually. Likewise, old devices that are no longer part of the network must be removed. An example of this type gateways is the one presented in reference \cite{Emara2009}. On the other hand, semi-automatic gateways can generate a link with the new IoT node but cannot automatically support the establishment of all configuration parameters \cite{Wu2013}. Finally, gateways that are fully automatic allow to self-configure new IoT devices and thus quickly solve heterogeneity problems during data transmission \cite{Kang2017}.

Next, some gateways that have been developed to improve interconnectivity between IoT devices will be described. For example, Gloria et al, in reference \cite{Gloria2017} describe the implementation of an IoT gateway that is the main component of a system dedicated to the monitoring and remote control of a pool. The gateway was developed using a Raspberry Pi board with full-duplex communication for data exchange between users and sensor networks. The sensors used in this platform are linked to an Arduino board which provides the connectivity to the gateway. The implemented sensors were: temperature, humidity, luminosity and level of water. However, data communication between the sensor network and the gateway is done through a USB cable. Thus, it is not feasible platform to implement in a real environment, due to the dependence of a wired connection.

Another gateway is the one proposed in \cite{Kang2018}, which is based on the IoTivity platform \cite{LinuxFoundation2019}. This gateway is focused on ensuring interoperability between devices with non-IP-based communication capabilities. To fulfill this objective, this gateway has implemented the CoAP (Constrained Application Protocol) protocol \cite{Shelby2014}. One of the advantages of this gateway is the self-configuration option, which allows a new sensor node to be connected to establish a dialogue with the gateway in order to be recognized as a new member of the system.

Other IoT gateways have been developed with the ESP32 card. For example, the implemented platform described in \cite{Khanchuea2019}, establishes a mesh network to data exchange between gateway and a sensor network. The sensor nodes use the DHT22 sensor to record temperature and humidity values. These nodes establish a ZigBee network to send the sensed data to a router node. This router node takes the data received by ZigBee link and relays it over WiFi to the gateway node. Although in this system there is a co-existence of two wireless networks (ZigBee and WiFi), the gateway node only establishes WiFi connections, so it lacks the property of being multiprotocol. 

Examples of multiprotocol gateways for IoT, can be consulted in references \cite{Guoqiang2013,YacchiremaVargas2016}. These gateways have as main function the conversion of protocols mainly between Zigbee, Bluetooth, WiFi and Ethernet. In these gateways data is stored and displayed through a web server embedded within the same gateway, which is not entirely practical if the possibility of a real application is analyzed. The most suitable would be the use of a cloud hosting service. 

According to the needs of the IoT ecosystem and the current needs of the IoT applications, we consider that an IoT gateway must have mainly the following characteristics:

\begin{itemize}
	\item Energy autonomy
	\item Multiprotocol
	\item Connectivity to Cloud Services
	\item Self-configuring
\end{itemize}

In next sections, we present an example of an IoT Gateway where some of the above features have been implemented. Also, we present a use case of the implemented gateway where a weather station with two wireless nodes transmit environmental data to the gateway. This data exchange between sensors nodes and gateway is simultaneously performed through three different communication protocols. Then, the IoT gateway delivers environmental data to a server in the Internet.

\section{A multiprotocol gateway for IoT: a proposed solution for the interoperability}
\label{sec:5.3}

A description of the architecture, hardware and software components of the developed IoT gateway will be given below. 
\subsection{Gateway architecture}

We have defined an architecture with five modules, which are summarized in Figure\ref{ch5_fig:3}. Each module is related to the main functions of the IoT gateway: (i) multiprotocol interconnection with remote nodes, (ii) data transformation, (iii) protocol conversion (iv) communication with IoT cloud platform and (v) user interface.

\begin{itemize}
\item Interconnection: the proposed architecture allows to interconnect several wireless nodes for data transmission, simultaneously, through different communication protocols (such as ZigBee, WiFi and Bluetooth). This communication is bidirectional, since the gateway collects data registered by wireless nodes through its sensors, but in addition, data can be sent to the nodes to operate on actuator devices.
\end{itemize}

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=0.8]{Figures/Fig3_Architecture}
\caption{Architecture of the developed IoT gateway}
\label{ch5_fig:3}       % Give a unique label
\end{figure}

\begin{itemize}
\item Data transformation: this module consists of standardization and establishment of a standard format to subsequently send data to a database server. This transformation is indispensable since data is sent from heterogeneous nodes that carried out the data capture through different types of sensors and that arrive through different network protocols. To standardize the representation of data, the JSON format was chosen, which has important advantages such as simplicity and low resource consumption. Also, a model is established for the identification of the devices that make up an IoT scenario. An example of the representation of the data recorded by the temperature and humidity sensor, in JSON format, is shown in Figure \ref{ch5_fig:4}. As can be seen in this figure, the first three fileds are "node-id", "gps" and "protocol", which correspond to the identification of the remote node, its gps coordinates and the protocol by which it transmitted the data. The following fields are "date", "sensor-id", "value" and "magnitude", which record the sensor information and its data. Finally, there is the “gate-id” and “network-id” fields, which will be used later to identify the gateway and the communication network. These last records will be useful when you have a scenario with more than one gateway and / or more than one transmission network.
\end{itemize}

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=1.0]{Figures/Fig4_Json}
\caption{Example of the standardized format for data transmission}
\label{ch5_fig:4}       % Give a unique label
\end{figure}

\begin{itemize}
\item Protocol conversion: the proposed IoT gateway acts as a bridge or translator between different protocols, mainly between ZigBee, Bluetooth, WiFi and Ethernet. Therefore, the gateway continuously must be listening for connection requests on its network interfaces. The reception of data by any communication protocol involves the extraction of the payload and the subsequent construction of a new message with the standardized format. For data transmission from the gateway to database server in the Internet, MQTT (Message Queuing Telemetry Transport) \cite{ISO2016} protocol is used. This protocol is recommended in network scenarios in which bandwidth consumption must be reduced and where the devices involved in communication have low processing and memory capacity. The MQTT protocol works under a publication-subscription model that uses three components: a Broker, a Subscriber and a Publisher. A device can be registered as a Subscriber to a topic of interest in order to obtain information published on that topic. The Publisher is the generator of data for a specific topic. Data of a topic are transmitted to the Subscriber through the Broker. Hence, a Broker can be considered as a server that routes messages published to Subscribers (see Figure \ref{ch5_fig:5}).
\end{itemize}

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=0.9]{Figures/Fig5_Mqtt}
\caption{Basic operation of MQTT protocol}
\label{ch5_fig:5}       % Give a unique label
\end{figure}

\begin{itemize}
\item Communication with IoT cloud platform: this module consists of receiving data from the sensors already formatted and sending them to an MQTT broker hosted on the Internet (iot.eclipse.org). It is also responsible for receiving the configuration parameters that a user can introduce through the graphical interface and transmit them to remote nodes, also using MQTT protocol. In the first case, communication from the gateway to the broker, the gateway uses the Eclipse Paho Python Client library and acts as a publisher. In the second case, that is, during the transmission from the gateway to wireless nodes, the gateway operates as a publisher and the wireless nodes as subscribers. Because wireless nodes (sensor nodes) do not have an Internet connection, it is also necessary that the gateway has a broker installed for this type of message exchange. The broker installed in the gateway was the well-known broker Mosquitto \cite{Light2017}, which due to its characteristics of low resource consumption and reduced overload information, is suitable for being installed on embedded boards. 
\item User interface: finally, the fifth module of the gateway allows user to introduce some system configuration parameters, through a graphical interface. Also, allows users to register new nodes and/or sensors, modification of the frequency of data capture rates, the assignment of communication protocols, visualization of the measures registered in the database, the creation of rules for announcements and alarms, among other functions.
\end{itemize}

It is important to clarify that in the proposed model, the database where the data is finally stored and the web platform where data can be displayed, are hosted outside the gateway, specifically, on a private server on the Internet.

\section{A multiprotocol gateway for IoT: a proposed solution for the interoperability}
\label{sec:5.4}

For the development of the gateway, the Samsung Artik 1020 development kit was used, which is a high performance and multi-protocol embedded board that has the possibility of wireless communications through Bluetooth, ZigBee and WiFi. It also has multiple I/O ports capable of communicating through I2C, SPI, UART modules. A summary with the main technical specifications is shown in Figure \ref{ch5_fig:6}.

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=0.8]{Figures/Fig6_Artik}
\caption{Main technical specifications of the Artik 1020 board}
\label{ch5_fig:6}       % Give a unique label
\end{figure}

\section{A multiprotocol gateway for IoT: a proposed solution for the interoperability}
\label{sec:5.5}

In order to evaluate the developed gateway architecture, a use case was built. The implemented system involves an IoT gateway and two remote wireless nodes. Each wireless node has 6 sensors registering the following variables: environmental temperature, relative humidity, solar radiation, wind speed, rainfall level and wind direction. The wireless nodes transmit data registered by sensors to the gateway through ZigBee, WiFi and Bluetooth. This data transmission was configured as follows: the wind direction and wind speed variables were transmitted using Bluetooth; the radiation variables and rainfall level through ZigBee; and finally, temperature and humidity over WiFi. A schematic diagram summarizing the use case implemented is shown in Figure \ref{ch5_fig:7}.

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=0.65]{Figures/Fig7_UseCase}
\caption{Use Case implemented}
\label{ch5_fig:7}       % Give a unique label
\end{figure}

The wireless nodes were implemented using the board Raspberry Pi 3 Model B with Ubuntu Mate as operating system. The sensors used were the following.

The sensor used to measure the ambient temperature and relative humidity is the AM2315. The Davis 6450 sensor is responsible for measuring solar radiation. And finally, the SEN-08942 kit was used, which consists of an anemometer, a rain gauge and a wind vane to determine the wind direction. A summary with the main characteristics of the wireless nodes is shown in Figure \ref{ch5_fig:8}.

\begin{table}[]
\begin{tabular}{|l|p{3.4cm}|l|p{1.2cm}|p{1.2cm}|p{2.0cm}|}
\hline \hline
\textbf{Model} & \textbf{Microcontroller} 										 & \textbf{Frequency} & \textbf{RAM} & \textbf{FLASH} & \textbf{SD Support} \\ \hline \hline
 Artik 1020    & Quad core ARM Cortex A15, Quad core Cortex A7 & 1.5 - 1.3 GHz      &  2 GB				 & 16 GB					& 32 Gb 									 \\ \hline
 Raspberry pi  & Broadcom BCM2837B0, Cortex-A53 64-bit         & 1.4 GHz						&  1 GB				 & 16 GB 					& 64 Gb 									 \\ \hline \hline
\end{tabular}
\caption{Main features of Artik and Raspberry Pi B+ boards}
\label{ch5_tab:1}       % Give a unique labe
\end{table}

Tables \ref{ch5_tab:1} and \ref{ch5_tab:2} show a comparison between the two embedded cards that were used for the implementation of the use case.

\begin{table}[]
\begin{tabular}{|l|l|l|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|p{1.2cm}|}
\hline \hline
\textbf{Model} & \textbf{Analog input} & \textbf{Digital I/O} & \textbf{UART} & \textbf{SPI} & \textbf{I2C} & \textbf{PWM} & \textbf{USB} \\ \hline \hline
Artik 1020     & 6 										 & 95 							 		& Si  					& Si  				 &	4						& 2						 & Si  					\\ \hline
Raspberry pi   & 0 							       & 48	  						 		& Si 						& Si 					 &	Si					&	2						 & Si					  \\ \hline \hline
\end{tabular}
\caption{I/O and Buses of Artik and Raspberry Pi B+ boards}
\label{ch5_tab:2}       % Give a unique labe
\end{table}

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=1.0]{Figures/Fig8_Node}
\caption{Use Case implemented}
\label{ch5_fig:8}       % Give a unique label
\end{figure}

\subsection{Sensors}

The sensor used to measure the environmental temperature and relative humidity was the AM2315 sensor. This has a humidity measurement accuracy of $\pm$ 2 \% and a temperature measurement of $\pm$ 0.1 C. Communication with the embedded system Raspberry pi is through the standard I2C protocol. In Figure \ref{ch5_fig:9} the mentioned sensor is shown. 

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=0.2]{Figures/Fig9_TempSensor}
\caption{AM2315 Sensor for environmental temperature and relative humidity}
\label{ch5_fig:9}       % Give a unique label
\end{figure}

On the other hand, for registration of the solar radiation, the Davis 6450 sensor was used. This transducer offers an analog output of 0 to 3Vdc, with a resolution of 1.67mV per W/m2 \cite{DavisInstruments2014}. In Figure \ref{ch5_fig:10} Davis 6450 sensor is exposed.

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=0.15]{Figures/Fig10_radiacion}
\caption{Solar radiation sensor}
\label{ch5_fig:10}       % Give a unique label
\end{figure}

Finally, the measuring kit SEN-08942, which has three different types of sensors to measure rainfall level, direction and speed of the wind. The rain gauge operates by momentary closing a switch every 0.011 inches (0.2794 mm) of rainwater collected in a bucket. These contacts are recorded with a counter activated by an interrupt input. An anemometer is used to measure the wind speed, a switch commanded by an encoder is activated for each rotation of the blades. Finally, weather vane is a combination of resistances which are used for measuring the wind direction through a voltage division \cite{SparkFunElectronics2009}. The measuring kit SEN-08942 is set forth below in Figure \ref{ch5_fig:11}.

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=0.5]{Figures/Fig11_estacion}
\caption{Weather station kit, SEN-08942}
\label{ch5_fig:11}       % Give a unique label
\end{figure}

\subsection{Data Analytic Tool}

The data analytic tool was developed to support client/server and publisher/subscriber communication architectures with the IoT gateway. It has an architecture by decoupled layers, with RESTful Web Service for communication between Backend and Frontend (see Figure \ref{ch5_fig:12}). The Backend has connection to MySQL 5.7 and MongoDB 4.2 databases through DAO and JPA, developed in JavaEE 7 on a Glassfish 4.1 server. For the connection with the broker, PAHO Eclipse 1.4 is used which publishes a Web Service with OAuth2 security to be consumed by the Frontend. The Frontend consumes the service with OAuth2 Client and a security token, the information is presented with Bootstrap chart according to the established data and variables.

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=1.0]{Figures/Fig12_analytic}
\caption{Architecture of the data analytic tool}
\label{ch5_fig:12}       % Give a unique label
\end{figure}

\subsection{Performance evaluation}

The performance evaluation of the monitoring system was carried out by recording the traffic received from the two wireless nodes through different communication protocols. The system implemented, performed data capture and transmission to the gateway for 8 minutes.Figure \ref{ch5_fig:13} and \ref{ch5_fig:14} show the throughput of the traffic received by the WiFi and Bluetooth interfaces, respectively, for each nodes. For WiFi traffic, it is observed that the aggregated traffic does not exceed 2.5 Kbps. On average, the traffic throughput of node 1 is 1.1 Kbps and for node 2 of 1.3 Kbps. These values are very low, despite that transmission frequency of the recorded variables was 6 seconds. With this low level of traffic, we can consider that there is still enough bandwidth to support the interconnection of more remote nodes without impact the traffic flows. In terms of traffic over Bluetooth, node 1 had an average throughput of 0.95Kbps and node 2 approximately 0.85Kbps. This is equivalent to approximately 1.8Kbps on average in aggregate traffic. Based on these values, with Bluetooth traffic, as with WiFi traffic, they show that more nodes could be added by transmitting to the gateway through this protocol. 

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=0.65]{Figures/Fig13_wifi}
\caption{Received Traffic over WiFi}
\label{ch5_fig:13}       % Give a unique label
\end{figure}

Similarly, Figure \ref{ch5_fig:15} shows the throughput achieve with ZigBee. The figure shows the aggregate traffic (node 1 + node2) and in this case, an average throughput of 16 Kbps was obtained. 

Finally, the percentage of CPU usage (see Figure \ref{ch5_fig:16b}) as well as the free memory were recorded (see Figure \ref{ch5_fig:16a}) every 10 seconds during system operation. That is, during the 8 minutes in which sensor nodes were transmitting environmental data to the gateway. Regarding CPU usage, the results show that only a 5\% of use was obtained. And in terms of RAM Memory, 1.5 GB of free memory was obtained on average, this represents an availability equivalent to 75\% of the total memory installed in the embedded board. The obtained results indicate that the processes implemented in the IoT gateway have a low consumption of resources, which would allow to incorporate more algorithms and more remote nodes simultaneously transmitting to the IoT gateway.

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=0.7]{Figures/Fig14_ble}
\caption{Received Traffic over Bluetooth}
\label{ch5_fig:14}       % Give a unique label
\end{figure}

\begin{figure}[hbt!]
%\sidecaption
\centering
\includegraphics[scale=0.65]{Figures/Fig15_Zigbee}
\caption{Received Traffic over ZigBee}
\label{ch5_fig:15}       % Give a unique label
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[scale=0.9]{Figures/Fig16_b_CPU}
\caption{Percentage of CPU usage}
\label{ch5_fig:16b}
\end{figure}

\begin{figure}[hbt!]
\centering
\includegraphics[scale=0.9]{Figures/Fig16_a_Memory}
\caption{Free RAM Memory}
\label{ch5_fig:16a}
\end{figure}

\subsection{Sensors Readings}

The following figures illustrate the sensors measurements for environmental temperature, relative humidity, wind speed and solar radiation. These variables were measured by wireless nodes for 7 minutes. Each figure has two curves which correspond to the measurements registered by the two nodes.

As shown in Figure \ref{ch5_fig:17}, the difference in temperature readings is not significant due to wireless nodes were located close to each other. Therefore, only a difference of 0.3 Celsius was registered.

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=1.0]{Figures/Fig17_temperature}
\caption{Environmental temperature readings}
\label{ch5_fig:17}       % Give a unique label
\end{figure}

Figure \ref{ch5_fig:18} Illustrates the relative humidity (in terms of percentage) measured by AM2315 sensors of both wireless nodes. The data variation is similar for the two nodes, obtaining a maximum difference in percentage of humidity of 1$\%$.

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=1.0]{Figures/Fig18_humidity}
\caption{Relative Humidity readings}
\label{ch5_fig:18}       % Give a unique label
\end{figure}

Figure \ref{ch5_fig:19} shows the measurements of wind speed taken by the kit SEN-08942. Nodes were in different places obtaining the value of the wind speed in Km/h. Therefore, readings have a similar variation in the two nodes.

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=1.0]{Figures/Fig19_sindSpeed}
\caption{Speed wind readings}
\label{ch5_fig:19}       % Give a unique label
\end{figure}

Finally, Figure \ref{ch5_fig:20} shows the solar radiation variable captured by Davis 6450 sensor, data is generated in $W/m^{2}$.

\begin{figure}[ht!]
%\sidecaption
\centering
\includegraphics[scale=1.0]{Figures/Fig20_Radiation}
\caption{Speed wind readings}
\label{ch5_fig:20}       % Give a unique label
\end{figure}

\section{Conclusions}
\label{sec:5.7}

In this chapter, we describe the technical impact of IoT as well the impact over the world economy. A discussion about the heterogeneity of IoT devices and the problems that this fact generates was also exposed. As a possible solution to interoperability problem caused by the heterogeneity of IoT devices we proposed a IoT gateway. The implemented gateway acts as the central element in a model in which several wireless nodes can send data through different communication protocols, such as: WiFi, Bluetooth, ZigBee and Ethernet. Acceptable results were obtained in the performance evaluation of the gateway in terms of bandwidth consumption as well as the percentage of CPU and RAM memory usage.

One of the main advantages of the proposed gateway is that it allows to configurate remote wireless nodes and data transmission to a data analytics service hosted on an Internet server. This provides flexibility in data storage and visualization.

\section*{Acknowledgements}
 This work is supported by the Universidad de San Buenaventura under the project “PIICO: Plataforma para la Interoperabilidad de dispositivos del Internet de las Cosas heterog\'eneos” (FI 014-006)

==> latexmkrc <==
$makeindex  = 'makeindex -s svind.ist %O -o %D %S';

# support for the glossaries package:
add_cus_dep('glo', 'gls', 0, 'makeglossaries');
add_cus_dep('acn', 'acr', 0, 'makeglossaries');
sub makeglossaries {
  system("makeglossaries \"$_[0]\"");
}

# support for the nomencl package:
add_cus_dep('nlo', 'nls', 0, 'makenlo2nls');
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}

# from the documentation for V. 2.03 of asymptote:
sub asy {return system("asy \"$_[0]\"");}
add_cus_dep("asy","eps",0,"asy");
add_cus_dep("asy","pdf",0,"asy");
add_cus_dep("asy","tex",0,"asy");

# metapost rule from http://tex.stackexchange.com/questions/37134
add_cus_dep('mp', '1', 0, 'mpost');
sub mpost {
  my $file = $_[0];
  my ($name, $path) = fileparse($file);
  pushd($path);
  my $return = system "mpost $name";
  popd();
  return $return;
}
